Optimal Multi-Agent Path Finding for Precedence Constrained Planning Tasks

Multi-Agent Path Finding (MAPF) is the problem of finding collision-free paths for multiple agents from their start locations to end locations. We consider an extension to this problem, Precedence Constrained Multi-Agent Path Finding (PC-MAPF), wherein agents are assigned a sequence of planning tasks that contain precedence constraints between them. PC-MAPF has various applications, for example in multi-agent pickup and delivery problems where some objects might require multiple agents to collaboratively pickup and move them in unison. Precedence constraints also arise in warehouse assembly problems where before a manufacturing task can begin, its input resources must be manufactured and delivered. We propose a novel algorithm, Precedence Constrained Conflict Based Search (PC-CBS), which finds makespan-optimal solutions for this class of problems. PC-CBS utilizes a Precedence-Constrained Task-Graph to define valid intervals for each planning task and updates them when precedence conflicts are encountered. We benchmark the performance of this algorithm over various warehouse assembly, and multi-agent pickup and delivery tasks, and use it to evaluate the sub-optimality of a recently proposed efficient baseline.

==> algorithms/expand_precedence_conflict.tex <==
\begin{algorithm}[t]
  \caption{ Expand Precedence Conflict}
%   \algorithmStyle
  \SetKwInOut{Input}{Input}
  \SetKwInOut{Output}{Output}
    \For{each constraint c in \{positive\_constraint,negative\_constraint\}}
    {
        positive\_constraint $\leftarrow$ robots $R_{p}$ collaborate on task $T_{q}$ at min(timestep\_set) \;
        negative\_constraint $\leftarrow$ robots $R_{p}$ do not collaborate  on task $T_{q}$ at min(timestep\_set)\;
        A $\leftarrow$ new node \;
        A.collaboration\_constraints $\leftarrow$ P.collaboration\_constraints + c \;
        A.collision\_constraints $\leftarrow$ P.collision\_constraints \;
        A.joint\_plan $\leftarrow$ P.joint\_plan \;
        \For{each agents $r_{i}$ in $R_{p}$}
        {
            invoke PC-CBS-lowLevelSearch for $r_{i}$ and update its plan in A.joint\_plan \;
        }
        A.cost $\leftarrow$ Makespan(A.joint\_plan)
        insert A in OPEN \;
    }
\end{algorithm}

==> inputs/07_ramification.tex <==
\subsection*{Ramifications} \label{subsec:discussion}

While PC-CBS has been proposed for precedence constrained tasks, the algorithmic framework can be adapted for other types of cross-schedule dependencies like synchronization and time-windowing constraints. Since the valid duration for tasks are represented by intervals, PC-CBS can integrate Safe-Interval Path Planning (SIPP) \cite{sipp} in its low-level search and be extended to continuous time domains similar to the work by \cite{ccbs}.  Recent work in improving CBS have significantly improved its run-time by choosing promising conflicts \cite{icbs}. Other works \cite{subopt_cbs} have proposed a highly efficient and bounded sub-optimal version of the algorithm. \cite{disjoint_cbs} found an order of magnitude improvement by incorporating positive constraints, which act as waypoints, to resolve collision conflicts in CBS. All of these improvements can be applied to PC-CBS, especially in the context of precedence conflicts.

% Another objective of this work is to inform better warehouse design, which is relevant to recent MAPF research \cite{bluesky}. Among the environments shown in Fig \ref{fig:environments}, the performance of H-CBS in warehouse assembly and collaborative MAPD problems is closer to the optimal paths in the Warehouse Grid environment than in the Maze environments. In typical warehouse applications like shown by \cite{life_mapd}, the MAPD problem is lifelong requiring dynamic planning. A fast algorithm which plans over segmented tasks is desirable in these cases. We provide the framework to calculate optimal solutions which can evaluate the sub-optimality of approximate solutions to these problems.

==> inputs/experiments.tex <==
\vspace{-3.2mm}


\section{Experimental Results} \label{sec:experiment}

We ran experiments on 9x9 grids in which agents could move from the center of one grid cell to the center of another. (Fig. \ref{fig:environments}). Cells colored black represent obstacles and cannot be occupied by any agents. At any timestep, an agent may either \textit{wait} at its current cell, or \textit{move} to its four-connected neighbourhood in the grid. The environments represent diverse scenarios for evaluation. The \texttt{empty-grid} does not contain any obstacles and provides large free spaces to agents for movement. The \textit{maze-tunnel} is highly constricted and requires passage through narrow tunnels to move between quadrants. 

In order to generate problems in different setups, we assigned random initial locations for each agent, and random pickup and delivery locations for transport tasks to create problems. The Task Graph edges, representing precedence constraints, are also randomly generated. Agents are allotted to their task sequences using a greedy assignment scheme. Among each task that can begin, we consider the set of agents that can reach it's start location. The task which can be started earliest is picked for allocation. This assignment strategy does not consider collisions between agents but it respects the precedence constraints between tasks. We run 100 different problem instances for each result and set the timeout for individual runs to 300s.

\input{inputs/tables/a2}

\subsection{Warehouse Assembly}

We define \textit{Warehouse Assembly} problems as a special class of PC-MAPF where precedence constraints form due to explicit inter-task dependencies. 

\subsection{Collaborative MAPD}

In \textit{Collaborative Multi-Agent Pickup and Delivery}, we consider situations where more than one agent is required to complete the transport tasks. Here, we do consider any scheduling order between different tasks. However, multiple agents have to arrive at the start location of the task forming implicit precedence constraints. 

\subsection{Tie-Breaking Heuristics}

In this section, we will evaluate the individual effects of the low-level heuristics defined in Algorithm 4. Specifically, we want to see which heuristics are key for the efficiency of the algorithm. To do this, we run 100 problems removing each heuristic one by one and compare the performance with the \textit{original} PC-CBS algorithm without any removals. Since removing the delay cost would make the algorithm sub-optimal, we replace it the normal \textit{f-value} heuristic to make the multi-waypoint A\* search admissable. For other heuristics, we can simply remove them from the vector. In addition to the number of problems solved, we report the mean time taken to solve the problems and the number of nodes expanded in the conflict tree of the search. The last two metrics are computed considering the problems solved by all three strategies for fair comparison.

\vspace{5mm}
\input{inputs/tables/a3}

Looking at the results on this PC-MAPF problem set, we observe that removing the \textit{count collisions} heuristic degrades performance most drastically. The amount of time taken by PC-CBS to find solutions without this heuristic is almost twice as much as with it. Removal of other heuristics have a smaller but still perceptible effect on performance. These effects are more pronounced in the tougher maze environments. This is expected because the \textit{empty} environment already has a lot of free space and the search does not require the aid of these heuristic values as much.

% We used a vector of tie-breaking heuristics within the low-level A* search in all of our previous experiments. In this section, we assess the value of employing this heuristic. We compare to a pure version of the algorithm that employs only one heuristic, the standard \textit{f-value} used in A*.
\subsection{Comparison to H-CBS}

We unify the implementations of PC-CBS and H-CBS algorithms in C++ using the Boost Graph library \cite{boost} for standard graph operations. Experiments are run on an Intel Core i7-1165G7 CPU @ 2.80GHz×8 processor with 15.3 GB of memory. we consider the practicality of scaling the PC-CBS and H-CBS to problems with higher number of mean tasks and agents. We show the trends in performance with changes in number of tasks and agents in the different environments.

\begin{figure}
    \centering
    \subfloat{{\includegraphics[width=0.45\linewidth]{images/comparison/pcmapf_agents.png} }}
    \qquad
    \subfloat{{\includegraphics[width=0.45\linewidth]{images/comparison/pcmapf_tasks.png} }}
    \caption{Scalability in Warehouse Assembly Problems}
    \label{fig:example}
\end{figure}

\begin{figure}
    \centering
    \subfloat{{\includegraphics[width=0.45\linewidth]{images/comparison/cmapd_agents.png} }}
    \qquad
    \subfloat{{\includegraphics[width=0.45\linewidth]{images/comparison/cmapd_tasks.png} }}
    \caption{Scalability in Collaborative MAPD Problems}
    \label{fig:example}
\end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{images/regret.png}
    \vspace{-0.7cm}
    \caption{\small {Surplus makespan, i.e, regret of H-CBS is visualized over the different gridworld environments using a Violin plot. The thick line in the middle indicates the mean regret. The problem set chosen here consisted of 6 agents with 3 mean tasks for both problem domains. The degree of collaboration is 2 for Collaborative MAPD.}}
    \label{fig:regret}
\vspace{-0.5cm}
\end{figure}

The amount of sub-optimality, however, is still significantly large in some case and shows the same variation with environments as shown in Fig \ref{fig:regret}. The problem sets where three agents collaborate for pickup tasks requiring three agents show no difference in makespan in any of the problems. This is expected since pre-emptive delays are never required in the case. Collaborative transport can start only when all agents arrive at the pickup location together. It is also observed that the performance of PC-CBS degrades quickly with increasing number of agents assigned to a task. For collaborative tasks, a cluster of conflicts can form around the pickup and delivery. Since the low-level search of PC-CBS employs a longer multi-waypoint search, the number of conflicts grows exponentially faster than in H-CBS.


% despite the availability of an open-sourced Julia implementation for H-CBS.

% \vspace{-20cm}
% \input{inputs/tables/2_degree_MAPD}
% \vspace{-20cm}
% \input{inputs/tables/3_degree_MAPD}
% \vspace{-2cm}

\vspace{-0.25cm}
\subsection{Extensions}
While PC-CBS has been proposed for precedence constrained tasks, the algorithmic framework can be adapted for other types of cross-schedule dependencies like synchronization and time-windowing constraints. Since the valid duration for tasks are represented by intervals, PC-CBS can integrate Safe-Interval Path Planning (SIPP) \cite{sipp} in its low-level search and be extended to continuous time domains similar to the work by \citet{ccbs}.  Recent work in improving CBS have significantly improved its run-time by choosing promising conflicts \cite{icbs}. Other works \cite{subopt_cbs} have proposed a highly efficient and bounded sub-optimal version of the algorithm. \citet{disjoint_cbs} found an order of magnitude improvement by incorporating positive constraints, which act as waypoints, to resolve collision conflicts in CBS. All of these improvements can be applied to PC-CBS, especially in the context of precedence conflicts. 

==> inputs/tables/a1.tex <==
% \usepackage{caption}
% \usepackage{multirow}


\begin{table*}[ht!]
\centering
\captionsetup{labelformat=empty}
\caption{\label{assembly}Performance Metrics in Warehouse Assembly Problems over 4 Different Grid Environments}
\label{assembly}
\vspace{-0.25cm}
\begin{tabular}{|c|c|l|c|c|l|c|c|l|c|c|l|c|} 
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Agents\\x Tasks\end{tabular}} & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Empty \\Grid\end{tabular}}                                                                                    & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Warehouse \\Grid\end{tabular}}                                                                                & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Maze-\\Gap\end{tabular}}                                                                                      & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Maze-\\Tunnel\end{tabular}}                                                                                    \\ 
\cline{2-13}
                                                                         & \begin{tabular}[c]{@{}c@{}}Succ.\\Rate\end{tabular} & \begin{tabular}[c]{@{}l@{}}Path\\Cost\end{tabular} & \begin{tabular}[c]{@{}c@{}}Time\\(s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Succ.\\Rate\end{tabular} & \begin{tabular}[c]{@{}l@{}}Path\\Cost\end{tabular} & \begin{tabular}[c]{@{}c@{}}Time\\(s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Succ.\\Rate\end{tabular} & \begin{tabular}[c]{@{}l@{}}Path\\Cost\end{tabular} & \begin{tabular}[c]{@{}c@{}}Time\\(s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Succ.\\Rate\end{tabular} & \begin{tabular}[c]{@{}l@{}}Path\\Cost\end{tabular} & \begin{tabular}[c]{@{}c@{}}Time\\(s)\end{tabular}  \\ 
\hline
2 x 2                                                                    & 1.00                                                & 30.0                                               & 0.1                                               & 1.00                                                & 31.3                                               & 0.1                                               & 1.00                                                & 33.2                                               & 0.1                                               & 0.99                                                & 33.8                                               & 0.8                                                \\
2 x 3                                                                    & 1.00                                                & 42.6                                               & 0.1                                               & 1.00                                                & 44.4                                               & 0.1                                               & 0.99                                                & 49.2                                               & 0.2                                               & 1.00                                                & 50.5                                               & 0.9                                                \\
2 x 4                                                                    & 1.00                                                & 56.4                                               & 0.3                                               & 1.00                                                & 59.7                                               & 0.3                                               & 1.00                                                & 62.2                                               & 0.6                                               & 0.99                                                & 68.2                                               & 2.1                                                \\ 
\hline
4 x 2                                                                    & 1.00                                                & 32.4                                               & 0.2                                               & 1.00                                                & 33.4                                               & 0.2                                               & 1.00                                                & 36.3                                               & 0.4                                               & 0.97                                                & 39.3                                               & 6.8                                                \\
4 x 3                                                                    & 1.00                                                & 50.3                                               & 1.4                                               & 1.00                                                & 51.6                                               & 2.5                                               & 0.99                                                & 54.0                                               & 2.5                                               & 0.89                                                & 59.4                                               & 10.1                                               \\
4 x 4                                                                    & 1.00                                                & 66.6                                               & 4.3                                               & 1.00                                                & 69.6                                               & 8.2                                               & 0.99                                                & 75.7                                               & 16.6                                              & 0.87                                                & 76.8                                               & 10.7                                               \\ 
\hline
6 x 2                                                                    & 1.00                                                & 33.4                                               & 0.7                                               & 1.00                                                & 35.1                                               & 1.2                                               & 0.99                                                & 36.8                                               & 4.7                                               & 0.89                                                & 39.8                                               & 15.4                                               \\
6 x 3                                                                    & 1.00                                                & 50.0                                               & 7.9                                               & 0.98                                                & 54.1                                               & 12.2                                              & 0.95                                                & 56.8                                               & 15.3                                              & 0.67                                                & 60.3                                               & 24.6                                               \\
6 x 4                                                                    & 0.99                                                & 72.0                                               & 15.9                                              & 0.95                                                & 72.9                                               & 26.7                                              & 0.84                                                & 78.1                                               & 45.2                                              & 0.52                                                & 78.7                                               & 46.5                                               \\ 
\hline
\multicolumn{1}{l}{}                                                     & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                               \\
\multicolumn{1}{l}{}                                                     & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                               \\
\multicolumn{1}{l}{}                                                     & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                               \\
\multicolumn{1}{l}{}                                                     & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                               \\
\multicolumn{1}{l}{}                                                     & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                               \\
\multicolumn{1}{l}{}                                                     & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                               \\
\multicolumn{1}{l}{}                                                     & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              
\end{tabular}
\vspace{-2.8cm}
\end{table*}

==> inputs/tables/a2.tex <==
% \usepackage{caption}
% \usepackage{multirow}


\begin{table*}[ht!]
\centering
\captionsetup{labelformat=empty}
\caption{\label{assembly}Performance Metrics in Collaborative MAPD Problems over 4 Different Grid Environments}
\label{assembly}
\vspace{-0.25cm}
\begin{tabular}{|c|c|l|c|c|l|c|c|l|c|c|lc|} 
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Agents x Tasks\\x Degree of\\Collab.\end{tabular}} & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Empty \\Grid\end{tabular}}                                                                                    & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Warehouse \\Grid\end{tabular}}                                                                                & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Maze-\\Gap\end{tabular}}                                                                                      & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Maze-\\Tunnel\end{tabular}}                                                                                    \\ 
\cline{2-13}
                                                                                               & \begin{tabular}[c]{@{}c@{}}Succ.\\Rate\end{tabular} & \begin{tabular}[c]{@{}l@{}}Path\\Cost\end{tabular} & \begin{tabular}[c]{@{}c@{}}Time\\(s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Succ.\\Rate\end{tabular} & \begin{tabular}[c]{@{}l@{}}Path\\Cost\end{tabular} & \begin{tabular}[c]{@{}c@{}}Time\\(s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Succ.\\Rate\end{tabular} & \begin{tabular}[c]{@{}l@{}}Path\\Cost\end{tabular} & \begin{tabular}[c]{@{}c@{}}Time\\(s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Succ.\\Rate\end{tabular} & \begin{tabular}[c]{@{}l@{}}Path\\Cost\end{tabular} & \begin{tabular}[c]{@{}c@{}}Time\\(s)\end{tabular}  \\ 
\hline
4 x 2 x 2                                                                                      & 1.00                                                & 27.0                                               & 0.6                                               & 1.00                                                & 29.2                                               & 4.1                                               & 1.00                                                & 31.5                                               & 4.2                                               & 0.99                                                & \multicolumn{1}{l|}{31.7}                          & 3.4                                                \\
4 x 3 x 2                                                                                      & 1.00                                                & 37.9                                               & 7.0                                               & 0.73                                                & 40.1                                               & 68.4                                              & 0.93                                                & 42.1                                               & 45.0                                              & 0.78                                                & \multicolumn{1}{l|}{43.6}                          & 51.0                                               \\ 
\hline
6 x 2 x 2                                                                                      & 1.00                                                & 28.2                                               & 3.4                                               & 0.83                                                & 29.6                                               & 29.3                                              & 0.96                                                & 31.1                                               & 19.3                                              & 0.84                                                & \multicolumn{1}{l|}{31.5}                          & 22.1                                               \\
6 x 3 x 2                                                                                      & 0.99                                                & 34.8                                               & 12.0                                              & 0.42                                                & 36.3                                               & 86.4                                              & 0.68                                                & 37.2                                               & 51.6                                              & 0.54                                                & \multicolumn{1}{l|}{37.6}                          & 57.7                                               \\ 
\hline
3 x 2 x 3                                                                                      & 1.00                                                & 29.0                                               & 1.3                                               & 1.00                                                & 29.7                                               & 1.7                                               & 1.00                                                & 30.8                                               & 3.6                                               & 1.00                                                & \multicolumn{1}{l|}{33.5}                          & 1.9                                                \\
3 x 3 x 3                                                                                      & 0.15                                                & 43.0                                               & 109.2                                             & 0.20                                                & 46.8                                               & 78.3                                              & 0.11                                                & 50.7                                               & 78.3                                              & 0.26                                                & \multicolumn{1}{l|}{55.2}                          & 78.3                                               \\ 
\hline
6 x 2 x 3                                                                                      & 0.93                                                & 28.6                                               & 28.7                                              & 0.72                                                & 30.2                                               & 63.9                                              & 0.73                                                & 32.2                                               & 55.9                                              & 0.65                                                & \multicolumn{1}{l|}{34.0}                          & 69.0                                               \\
6 x 3 x 3                                                                                      & 0.20                                                & \multicolumn{1}{c|}{36.0}                          & 124.6                                             & 0.13                                                & \multicolumn{1}{c|}{39.8}                          & 121.4                                             & 0.13                                                & \multicolumn{1}{c|}{36.5}                          & 134.4                                             & 0.12                                                & \multicolumn{1}{c|}{45.7}                          & 110.6                                              \\ 
\hline
\multicolumn{1}{l}{}                                                                           & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                &                                                    & \multicolumn{1}{l}{}                               \\
\multicolumn{1}{l}{}                                                                           & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                &                                                    & \multicolumn{1}{l}{}                               \\
\multicolumn{1}{l}{}                                                                           & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                &                                                    & \multicolumn{1}{l}{}                               \\
\multicolumn{1}{l}{}                                                                           & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                &                                                    & \multicolumn{1}{l}{}                               \\
\multicolumn{1}{l}{}                                                                           & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                &                                                    & \multicolumn{1}{l}{}                               \\
\multicolumn{1}{l}{}                                                                           & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                &                                                    & \multicolumn{1}{l}{}                               \\
\multicolumn{1}{l}{}                                                                           & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                & \multicolumn{1}{l}{}                               & \multicolumn{1}{l}{}                              & \multicolumn{1}{l}{}                                &                                                    & \multicolumn{1}{l}{}                              
\end{tabular}
\vspace{-2.8cm}
\end{table*}

==> inputs/tables/a3.tex <==
% \usepackage{caption}
% \usepackage{multirow}


\begin{table}
\centering
\captionsetup{labelformat=empty}
\caption{\label{assembly}Heuristics Ablation Study: We evaluate the effect of the tie-breaking heuristics on different problem sets in the Warehouse Grid environment}
\label{assembly}
\begin{tabular}{|c|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Agents\\x Tasks\end{tabular}} & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}PC-CBS\\(Tie-Breaking)\end{tabular}}                                                                           & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}PC-CBS\\(Vanilla)\end{tabular}}                                                                                 \\ 
\cline{2-7}
                                                                         & \begin{tabular}[c]{@{}c@{}}Succ.\\Rate\end{tabular} & \begin{tabular}[c]{@{}c@{}}Nodes\\Exp.\end{tabular} & \begin{tabular}[c]{@{}c@{}}Time\\(s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Succ.\\Rate\end{tabular} & \begin{tabular}[c]{@{}c@{}}Nodes\\Exp.\end{tabular} & \begin{tabular}[c]{@{}c@{}}Time\\(s)\end{tabular}  \\ 
\hline
2 x 3                                                                    & 1.00                                                & 1.6                                                 & 0.10                                              & 1.00                                                & 2.1                                                 & 0.14                                               \\
2 x 4                                                                    & 1.00                                                & 1.6                                                 & 0.25                                              & 1.00                                                & 2.2                                                 & 0.38                                               \\
4 x 3                                                                    & 1.00                                                & 5.5                                                 & 1.4                                               & 0.98                                                & 12.3                                                & 4.1                                                \\
4 x 4                                                                    & 1.00                                                & 5.1                                                 & 5.4                                               & 0.93                                                & 12.2                                                & 18.2                                               \\
6 x 3                                                                    & 0.98                                                & 9.1                                                 & 5.1                                               & 0.82                                                & 34.9                                                & 22.9                                               \\
6 x 4                                                                    & 1.00                                                & 12.2                                                & 15.7                                              & 0.78                                                & 32.0                                                & 56.9                                               \\ 
\hline
\multicolumn{1}{c}{}                                                     & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                              & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                               \\
\multicolumn{1}{c}{}                                                     & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                              & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                               \\
\multicolumn{1}{c}{}                                                     & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                              & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                               \\
\multicolumn{1}{c}{}                                                     & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                              & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                               \\
\multicolumn{1}{c}{}                                                     & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                              & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                               \\
\multicolumn{1}{c}{}                                                     & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                              & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                               \\
\multicolumn{1}{c}{}                                                     & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                              & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                                & \multicolumn{1}{c}{}                              
\end{tabular}
\vspace{-2.8cm}
\end{table}

==> inputs/tables/heuristics_results.tex <==
% \usepackage{caption}
% \usepackage{multirow}


\begin{table}[h]
\centering
\caption{\label{h_pcmapf}Ablation Study: We removed one element at a time from the vector of heuristic defined by Alg. 4 and test on a set of PC-MAPF problems with 4 agents and 2 mean tasks }
\label{h_pcmapf}
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{|c|ccc|ccc|ccc|ccc|} 
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Heuristic\\Mode\end{tabular}} & \multicolumn{3}{c|}{Empty Grid}                                                                               & \multicolumn{3}{c|}{Warehouse Grid}                                                                           & \multicolumn{3}{c|}{Maze-Gap}                                                                                 & \multicolumn{3}{c|}{Maze-Tunnel}                                                                               \\ 
\cline{2-13}
                                                                         & Sol. & \begin{tabular}[c]{@{}c@{}}Time\\(s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Node\\Exp.\end{tabular} & Sol. & \begin{tabular}[c]{@{}c@{}}Time\\(s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Node\\Exp.\end{tabular} & Sol. & \begin{tabular}[c]{@{}c@{}}Time\\(s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Node\\Exp.\end{tabular} & Sol. & \begin{tabular}[c]{@{}c@{}}Time\\(s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Node\\Exp.\end{tabular}  \\ 
\hline
Original                                                                 & 1.00 & 0.22                                              & 2.1                                                & 1.00 & 0.42                                              & 5.1                                                & 1.00 & 0.42                                              & 5.8                                                & 0.98 & 0.46                                              & 8.4                                                 \\
No delay                                                                 & 1.00 & 0.22                                              & 2.2                                                & 1.00 & 0.45                                              & 5.1                                                & 1.00 & 0.50                                              & 6.8                                                & 0.97 & 0.52                                              & 8.9                                                 \\
No colab                                                                 & 1.00 & 0.22                                              & 2.1                                                & 1.00 & 0.45                                              & 9.6                                                & 1.00 & 0.48                                              & 5.8                                                & 0.98 & 0.48                                              & 8.4                                                 \\
No collision                                                             & 1.00 & 0.48                                              & 4.5                                                & 0.99 & 0.89                                              & 5.1                                                & 0.99 & 2.45                                              & 21.8                                               & 0.94 & 2.99                                              & 42.3                                                \\
No move                                                                  & 1.00 & 0.17                                              & 2.1                                                & 1.00 & 0.31                                              & 5.0                                                & 1.00 & 0.36                                              & 5.7                                                & 0.98 & 0.37                                              & 8.5                                                 \\
\hline
\end{tabular}
\end{adjustbox}
\end{table}
